Demand-side management via optimal production scheduling in power-intensive industries: The case of metal casting process

The increasing challenges to the grid stability posed by the penetration of renewable energy resources urge a more active role for demand response programs as viable alternatives to a further expansion of peak power generators. This work presents a methodology to exploit the demand flexibility of energy-intensive industries under Demand-Side Management programs in the energy and reserve markets. To this end, we propose a novel scheduling model for a multi-stage multi-line process, which incorporates both the critical manufacturing constraints and the technical requirements imposed by the market. Using mixed integer programming approach, two optimization problems are formulated to sequentially minimize the cost in a day-ahead energy market and maximize the reserve provision when participating in the ancillary market. The effectiveness of day-ahead scheduling model has been verified for the case of a real metal casting plant in the Nordic market, where a significant reduction of energy cost is obtained. Furthermore, the reserve provision is shown to be a potential tool for capitalizing on the reserve market as a secondary revenue stream.

==> Framework.tex <==
The following section presents the methodological approach to deal with the demand-side management of intensive industrial consumers.%, by which they can gain benefits for its application in a context of liberalized energy markets.
The energy-aware scheduling components are framed in the overall picture of different interacting modules required for a complete and effective application of industrial demand response strategies.\\% The link among these components and the various electricity markets is also shown.\\
After a general presentation of these topics, the approach is particularized for the case of a metal casting process. 
\subsection{Tools for Energy-Aware Scheduling}%Framework}
The application of industrial Demand Response is made possible by the implementation of a composite tool set, among which  the Energy-Aware Scheduling (EAS) is the fundamental element.  Nevertheless, a brief description of the overall system is given, to provide the reader a general understanding of it.
%
\begin{figure}[!ht]
	\centering
	%\includegraphics[width=0.65\linewidth]{Schema_1}
	\scalebox{0.4}{ \input{Schema_1.eps_tex}}
	\caption{Comprehensive framework to support industrial Demand Response. The scheme shows the interaction of the different items for iDR (in red) and the coupling with the corresponding electricity market (in green), highlighting the time framework in which each tool operates. Price Forecast (PF) blocks are required to provide foreseen costs and revenues. The Sequential EAS modules, which are the core of the paper, are framed in the grey box}
	\label{fig:DR_framework}
\end{figure}
%
%
Figure~\ref{fig:DR_framework} draws the essential components, showing the interaction among other them and the connections to the electricity market.
This framework is composed by modules that convert the short term production plan, received from the Enterprise Resource Planning (ERP) layer, in to the task schedule that minimizes the energy cost at the same throughput level. This is achieved taking into consideration the interplay with the electricity prompt market. %Eventually, it compensates for disturbances and deviations in real time.
%up to the controlled execution on the shop-floor. 
The production plan is assumed to be related to the electricity delivery period.\\%, in general 24 hours starting at midnight.\\
It is important to note that these components operate in different time frames and they are linked to distinct electricity markets.
Referring to Figure~\ref{fig:DR_framework}, two regions can be defined:
%The scheme shows two main parts based on the time frame in which the components operate and on the mechanisms of the electricity market: 
i) the \textit{scheduling} zone, containing modules that work during the %\txtred{ex-ante spot market | trading period}
auction period, when the production is not yet started; ii) the  \textit{execution} region, in which modules run during the delivery period, when the production is in progress.%, considering the horizon of the production plan 
In the first zone, our framework differentiates among scheduling steps that are not market related, as Batch Sequencing and Line Allocation (BS-LA), and the actual EAS steps, which are connected to the electricity market.\\
The very first step of the scheduling procedure is performed by BS-LA, where the aggregated orders of the production plan are decomposed in manageable batches, allocated among the multiple production lines and sequenced. This can be typically modelled as multi-machine flow shop scheduling problem and solved with a Mixed Integer Linear Programming method.\\
The list of ordered jobs is then provided as input to the EAS system that computes the optimal scheduling considering energy related aspects and constraints: in particular, but not limited to, time-varying energy prices, energy and power constraints associated to the process or to the specific demand response programme.

All the modules of the first region utilize deterministic models of the process, i.e. they consider nominal execution times and capacities, as well as theoretical energy targets for each job. 
Nevertheless, in the class of problems examined, possible stochastic elements that can influence the energy requirements of a job exist, e.g. %these are mainly 
related to the varied distribution of raw material qualities. In the proposed framework, these issues are managed during the execution phase by  the Receding Horizon Real-Time (RHRT) system.\\
During the delivery period, the Receding Horizon Real-Time component enforces the consumption of the committed energy profile. The RHRT considers a sub-horizon of the delivery day, in which it compensates for any variation between the actual and the committed energy, refining the schedule or trading energy deltas on the imbalance market. Such variations %between actual and committed energy profiles 
may in fact depend on a different effective value of the job energy target, which %can be influenced by 
is a stochastic processes. In order to deal with this, the RHRT operates cyclically in a receding horizon fashion, shifting forward the optimization window and compensating for unforeseen variations.



\subsection{Market}\label{subsec:Market}
The current paper focus on a distinctive EAS, defined as Sequential EAS.%, shown in Figure~\ref{fig:DR_framework}.
Its objective is to operate in a industrial Demand Response scenario, in which the production flexibility is exploited primarily in the non-dispatchable maket and secondarily in a dispatchable one.%electricity market. 
In the process of developing DR strategies, in this work, we have tried to keep related models general in terms of market specifications such as clearing mechanisms, gate closure and time intervals.  However, when it is necessary to make assumptions we have adopted the rules of Danish market, which is eventually used for the case study.   
The non-dispatchable, or implicit, energy market considered here is the Day-Ahead (DA) market, where electricity supply/demand is traded for each hour of the next day. A forecast of the next day hourly prices is used to minimize the energy cost required to fulfil the production plan. 
The dispatchable, or explicit, market is instead a Reserve Capacity (RC) market. The reserve capacity is the share of power that might be used, upon TSO request, to cover imbalances between generation and load on the grid, due to random variations in demand or production. A positive and a negative reserve power can be offered for every time slot.% on the RC market. 
The market rewards the committed availability of a reserve capacity, regardless of its actual activation. The duration of the reserve and the maximum number of potential daily requests are market-dependent.
To participate in a RC market, a reference profile is needed: our framework - defined for this reason Sequential EAS - considers the energy curve committed in the previous EAS step (DA market) as baseline.

\txtred{ $\Downarrow$ THIS PART MUST BE REVIEWED}
In Nord pool exhange market, it is possible to participate in the auction either offering a bidding curve or independently from the price just by an hour-specific volume demand.
\txtred{ With a price independent order for all hours, the member will receive a schedule of deliveries equal to the specified volume for all hours, regardless of the price level within the range.}\\ 
If a process (like the one studied by Xang) \txtred{CHANGE REF STYLE} can be characterized by profitability without long-term delivery commitments, it can hedge against price uncertainty via price-dependant bid (bidding curve). However, in process with binding daily production plan (which corresponds to a certain daily energy consumption) it is not possible to participate in the auction with different price-volume pairs as the final cleared quantity may not be sufficient for fulfilling production commitments. Thus such customers may prefer to participate in the market through an aggregator whose would be responsible for price risk mitigation.
\txtred{role of the aggregator and mechanism of shadow prices}. If the end user (foundry) is connected to market (whether it be energy or capacity ) via aggregator/broker/retailer it may require that several load profiles to be generated in response to a shadow price that is sent by the aggregator for balancing and hedging purposes. In that case a faster optimization is required. Such a scheme is not in the scope of this work. \txtred{will be discussed in the paper with VITO} 
\txtred{In the next section, it is shown the application of this Energy-Aware framework to the iron casting case study. }

==> Introduction.tex <==
\section{Introduction: \\
The role of energy-intensive industries}

The last decade has witnessed a major paradigm shift in EU energy market and policies. On one hand the electricity market was deregulated in order to increase competition thus decrease the prices, on the other hand EU has made the commitment to a 20\% reduction of its Greenhouse gas emission by 2020 through increase in the share of renewable energy in the final energy consumption.\\
In order to facilitate the penetration of renewable energy sources mechanisms are needed to be in place to deal with unresponsiveness of these sources to system demand due to their intermittent nature. Such mechanism should be able to ensure grid reliability in delivering the user's exact demand at any time and maintain its operational security by compensating any imbalance between power in-flows and out-flows which could cause blackouts. \\ 
An straightforward remedy to these challenges would be the installation of storage systems to store energy during the production peaks (i.e. sunny or windy hours) and dispatch them during the demand peaks. However this requires huge investment on energy efficient storage system which is not realistic for the near future\\
A more practical approach which of high interest to grid operators is to engage the end users or their agents in a power balancing scheme in order to shape the consumption pattern by exploiting their demand flexibility. Techniques involving such practices are referred to as Demand-Response or Demand-Side Management. \\
\txtred{arg1}
There are two main classes of DSM strategies to motivate the user to change its load curve [ref?]:\\
\textit{Incentive-based programs:} is an explicit participation of customers in which they choose to give the grid operator (\txtred{TSO}) control over their non-crucial electricity load in return for a compensation. Although the price-based methods are more desired by TSO because of their guaranteed availability, it is may not be well suited for some industrial users with less certainty in their underlying process and more strict delivery commitments.\txtred{(some drawbacks making it not suitable for steel industry)}\\
\textit{Price-based programs:} is an implicit demand-side participation characterised by volunteer response of the end user to time-varying electricity tariffs set by \txtred{TSO/BRP}. There are different programs of these type based on the response time-scale:
\begin{enumerate}[1)]
	\item Time of Use (TOU)[Year(s)/month ahead]: \txtred{definition}
	\item Day-ahead hourly pricing: 
	\item Real-time/critical peak pricing:  
\end{enumerate}
   
\txtred{Role of TSO, BRP, aggregatore...}\\

How aggregator would allow 



\txtred{incentives for participation: users benefit} 
\txtred{other benefits: potential for further reduction in C02 by changing the consumption pattern of the systems with high polluting peaks, helping the market system to increase its competitiveness in long term by increasing the price margin considering the production cost }   

role of energy-intensive industries

Energy-intensive industries with enough flexibility in power and significant energy consumption are particularly appropriate for the demand side management. \citep{Paulus2011} proposed two criteria to identify the sectors with the greatest economic potential for implementation of DSM: high electricity demand and high specific costs for electricity.  That study gave prominence to five processes: cement mills, inorganic material and chemical processes, aluminium electrolysis, paper industry and iron and steel plants.\\
Examples of application of EES to various energy-intensive industries can be found in literature: \citep{Mitra2012} discussed the modification of the production schedule to include energy for the case of air separation plants, \citep{Castro2009} present a Resource Task network (RTN) formulation suitable for a continuous plant and applied to the grinding stage of a cement plant, while an alternative approach based on robust optimization is presented in \citep{Vujanic2012} for a the process od crushing rocks in a cement production chain.


Power supply and demand must balance in any time: energy-intensive industries can play an important role in the reliability of the grid, providing the required stability and flexibility, \citep{Paulus2011}. 
Demand Side Management (DSM), in particular Demand Response, is a way to contribute to enanched energy management, shaping the energy demand profile acting on the consumer side, based on different methods and approaches \citep{Palensky2011}.\\
Usually demand response is limited to emergency load relief and peak load reduction, but as shown by \citep{Ma2013}, DSM has also proven its economic value and the impact on the electrical system as a resource to provide ancillary services, in particular for the tertiary reserve.
Demand response strategies are capable of enhancing reliable operation of energy grid with faster response time and lower costs
with respect to traditional generation utilities \citep{Shoreh2016}.\\
Smart energy management is becoming a key factor in the current and future industrial scenario, not only for systemic grid reliability but also for sustainability and operational profitability. The latter, in energy-intensive industrial processes, can be increased through advanced production management under time-varying energy pricing, where the revenues can come directly from a reduction of operational costs and not just from selling DSM services.\\
Energy-aware scheduling (EAS) \citep{Merkert2014}, or as defined by \citep{Gahm2016} energy-efficient scheduling (EES), is a proper tool to provide these benefits, improve energy efficiency and optimize energy usage.\\



\txtred{In this paper we...}\\

In the rest of this paper first we are going to review previous works regarding industrial demand side management both in explicit and implicit framework. Then a brief description of the problem in hand is given in section ?? where foundry process is explained. Furthermore, market mechanism ,participation requirements and barriers are discussed in sec ??? for subsequent consideration in the modelling. In sec ?? melting and casting process are modelled and technical and operational constraints are translated to MILP form. This modelled is then incorporated into a price-based demand response optimization (sec ??) which also sets a baseline that is used later as the reference power profile within an incentive-based DR optimization.  

In this framework the implicit programme is considered to be the main profitability engine as energy is main commodity of interest for an energy-intensive process. Another reason is the nature of those markets. Comparing to wholesale energy market, the amount traded in capacity market is much lower which makes the acceptance of eventual bids ... \txtred{barriers of participation in the capacity market }
It is important to notice that in both cases we assume the energy price in both day-ahead and balancing (regulating) market is predictable with a good accuracy which we define as close timing of peak and valleys and  

\txtred{is not in the scope of this paper}\\


\section{Literature review}


Several works address the steel industry: \citep{Nolde2010} focus on the scheduling solution to track a predefined load, \citep{Hait2011, Artigues2013} dedicate to the same problem, modifying the treatment of binary variables in order to improve the computational performance; \citep{Castro2013} formulate an approach for production scheduling under energy constraints in a steel plant.
\citep{Ashok2006} concentrate on a discrete time formulation for peak load management of mini steel plants in a scenario of time of use (TOU) tariff, instead \citep{KamaraEsteban2012} approach the problem of energy-aware production scheduling of a foundry using genetic algorithms and simulating annealing.\\ 
The present paper addresses the scheduling of a foundry melt shop, focusing on the energy-aware scheduling of induction furnaces, since the melting process employs almost 80\% of the electricity consumption of the plant \citep{Lazzarin2015}.
The approach described in this work applies to the typical configuration of an iron casting foundry, the most energy efficient \citep{Schmitz2014}, that comprises a set of coreless induction furnaces (IF) for melting and channel induction furnaces for holding the metal before casting.
Every furnace can be in general different, by capacity, energy model and efficiency. Subsets of furnaces can be coupled by a constraint on the resource, representing a single power unit serving all of them, while a global time-varying constraint on the power is imposed on the entire plant, as well as a time-varying price of the shared resource. Maximum deadlines are defined for every job by an higher level system.
\citep{Hait2007, Hait2009} present a continuous-time approach to the energy scheduling problem on a similar application, including operator availability. Their approach is non-preemptive and it assumes known span for loading and unloading phases, while the duration of the melting stage depends directly on the consumption of the resource. In the first paper, the authors highlight the limitation of a discrete-time approach of the scheduling problem, as proposed in \citep{Trepanier2005}, because the huge number of binary variables made it impossible to tackle realistic problems.\\
The innovative approach presented in this paper, can overcome the limitations of discrete-time schemas: thanks to a receding horizon decomposition and a tighter optimization problem, the algorithm can handle real-world problems effectively.\\
The model formulation has special features and specific constraints due to the peculiarity of the application. At the same time, however, with some relaxation it can be generalized to the scheduling of a batch process on parallel machine with resource and capacity constraints under time-varying resource pricing, where tasks have to be processed within defined release and due dates. It can be classified as an extension of a preemptive resource-constrained project scheduling problem (RCPSP), similar to its multi-mode variant (MRCPSP) \citep{Hartmann2010}. The continuously-divisible renewable resource, as defined by \citep{Brucker1999}, has limited capacity. However, this scheduling problem cannot be solved with the numerous classical variants of the RCPSP, since resource request and task duration are inter-dependent and it can vary within task duration. The peculiarity of this class of problems is that the task is completed when a certain amount of cumulative resource is provided. Thus, the duration of a task depends on the resource capacity and the resource intensity assigned to it.\\


 


















